Towards a first design of a Newtonian-noise cancellation system for Advanced LIGO

Newtonian gravitational noise from seismic fields is predicted to be a limiting noise source at low frequency for second generation gravitational-wave detectors. Mitigation of this noise will be achieved by Wiener filtering using arrays of seismometers deployed in the vicinity of all test masses. In this work, we present optimized configurations of seismometer arrays using a variety of simplified models of the seismic field based on seismic observations at LIGO Hanford. The model that best fits the seismic measurements leads to noise reduction limited predominantly by seismometer self-noise. A first simplified design of seismic arrays for Newtonian-noise cancellation at the LIGO sites is presented, which suggests that it will be sufficient to monitor surface displacement inside the buildings.

==> optimal_old.tex <==
\section{Array Optimization}
\label{sec:optimization}

There are different methods to find the optimal array, which are all based on minimizing eq.~(\ref{eq:R}). The method used in \cite{Har2015} first applies analytic transformations of the equation to determine the optimal array as zeros of a new set of equations. Alternatively, one can directly find the minimal residual by applying generic high-dimensional sampling algorithms such as nested sampling, Metropolis Hastings MCMC, or particle swarm optimization (the last was used in \cite{DHA2012}). 

The results in this paper were calculated with a Metropolis Hastings MCMC algorithm implementing adaptive simulated annealing (SA), which statistically guarantees obtaining solutions close to global minima \cite{Kirkpatrick671,Ingber_ASA}. The cost function involves a parameter space with dimensionality $2N$ (for $N$ sensors)  with numerous local minima.  The algorithm should optimize all seismometer locations simultaneously to obtain near to global solutions within a reasonable execution time. SA is a probabilistic method whose name draws inspiration from a metallurgic annealing process where heating followed by slow cooling results in achieving minimum energy configuration in a crystal lattice . The success of the optimization depends on careful selection of the probability distribution $g_{T}(x)$ used to span the multi-dimensional parameter space, acceptance criteria $h(\Delta{E})$ are used to select the newer points and the temperature or the annealing schedule, which determine the level of vigorousness associated with the search.  Algorithm is constructed to begin as a random exploration of the parameter space and then progress with time towards a greedy search. 

Usually the acceptance function is given by $h(\Delta{E}) = 1/(1+\Delta{E}/T)$ where $\Delta{E}$ is the difference in cost function between the new and the previous state. The state space probability distribution is given by a Cauchy distribution $g(\Delta{x}) = T/(\Delta{x}^{2} + T^{2})^{(D+1)/2}$. The exponential annealing schedule is used to calculate temperature at future time steps $T_{i}(k) = T_{0i}\; \exp (c_{i} k^{1/D} ) $ with $c_{i} = m_i \; \exp(-n_i/D)$. Here $m_{i}$ and $n_{i}$  act as free parameters that are used to fine tune the optimization process.  

The variation in sensitivities of different parameters during the course of the search is addressed by reannealing or rescaling the time-steps after every user-defined number of accepted states. This essentially  decreases or increases the range for those parameters, which show more or less sensitivity at the current annealing schedule. Accuracy of the search after each SA iteration is further enhanced by performing a polling based pattern search, which is well suited for carrying out local minimization when the problem at hand is ill-defined and non-differentiable.  In our implementation, we perform parallel analysis at each iteration by executing a MATLAB implementation of adaptive SA  on different computing cores and selecting the best configuration for  use in further iterations.  Here the annealing schedule and the process of newer samples generation get adaptively modified so as  to achieve accelerated convergence.

For optimizing the array locations, the algorithm is as follows. We will use either the analytic or measured seismometer correlations, denoted $C_{\rm SS}$. Arrays with $N$ seismometers are then generated by the algorithms. The $C_{\rm SS}$, and thereby the $C_{\rm SN}$ using eq.~(\ref{eq:correlations}), is then computed for the various cases of seismic correlations. This process is repeated until the algorithm's stopping criterion is reached, and thereafter the array with the smallest residual is taken to be the optimal array.

We make a number of assumptions in the following analysis. First, since seismic fields are highly stationary in the 10 -- 20\,Hz range at the LIGO sites \cite{Har2015}, arrays are optimized towards maximal reduction of a stationary NN background. It is possible that rare strong transients in the 10 -- 20\,Hz range are better suppressed by arrays with different configurations. Second, we assume a signal-to-noise ratio (SNR) of 100 for the seismic sensors. In low-noise environments such as underground sites even the most sensitive seismometers do not necessarily achieve SNRs of 100 in the NN band, but at the existing sites of the LIGO and Virgo detectors with seismic spectra being a few orders of magnitude above the global low-noise model \cite{Har2015}, the most sensitive instruments in the NN band such as GS-13, STS-2, or T240 have SNRs of a few 1000, and relatively inexpensive sensors already have SNRs of a few 100. Third, we choose for the test mass to be suspended 1.5\,m above ground, which is approximately the height of the LIGO test masses. It should be noted though that the test-mass height has no effect on optimal arrays for cancellation of NN from plane-wave Rayleigh fields. In our simulation, we search for optimal sensor locations within a 100\,m $\times$ 100\,m surface area with a test mass at its center. This is conservative, as this is larger than the area from which interesting NN contributions are expected \cite{HaEA2009a}. 

